ScatterShot: Interactive In-context Example Curation for Text Transformation

The in-context learning capabilities of LLMs like GPT-3 allow annotators to customize an LLM to their specific tasks with a small number of examples. However, users tend to include only the most obvious patterns when crafting examples, resulting in underspecified in-context functions that fall short on unseen cases. Further, it is hard to know when "enough" examples have been included even for known patterns. In this work, we present ScatterShot, an interactive system for building high-quality demonstration sets for in-context learning. ScatterShot iteratively slices unlabeled data into task-specific patterns, samples informative inputs from underexplored or not-yet-saturated slices in an active learning manner, and helps users label more efficiently with the help of an LLM and the current example set. In simulation studies on two text perturbation scenarios, ScatterShot sampling improves the resulting few-shot functions by 4-5 percentage points over random sampling, with less variance as more examples are added. In a user study, ScatterShot greatly helps users in covering different patterns in the input space and labeling in-context examples more efficiently, resulting in better in-context learning and less user effort.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> appendices/clusters.tex <==
\section{Clustering for \qa}
\label{appendix:qa_cluster}

\begin{figure*}[h]
\centering
\includegraphics[trim={0cm 18cm 16cm 0cm}, clip,width=1\linewidth]{figures/slice_qa.pdf}
\vspace{-15pt}
\caption{
A demonstration of the sampling procedure for \qa.
}
\vspace{-10pt}
\label{fig:slice_qa}
\end{figure*}

==> backups/method.tex <==
\section{\sysname: Design and Implementation}

\subsection{Design Considerations}
The goal of \sysname is to help human annotators find appropriate examples for specifying their desired in-context functionality.
An example would be ``appropriate'' if it helps to:
%\textbf{specify function applicability and intended behaviors}.


%As explained in Section~\ref{scattershot:sec:intro} and Figure~\ref{scattershot:fig:teaser}, the objective of \sysname is to help users appropriately specify their desired in-context functionality. 
%We design our method to aid humans in the following two dimensions: 

\begin{enumerate}[nosep,labelwidth=*,leftmargin=1.8em,align=left,label=D.\arabic*]

\item \label{scattershot:sample:negative} \textbf{Specify function applicability}.
Because LLMs are generative in nature, they would try to produce the most plausible ``label'' even for negative examples~\cite{sobieszek2022playing}.
For example, in Figure~\ref{scattershot:fig:teaser}, LLM attempts to normalize \exinline{5\%} to a most plausible \exinline{1988} even though there is no date in the sentence.
This implies that we need to explicitly specify negative examples in the training set, so as to guide LLMs to avoid undesired hallucinations.

\item \label{scattershot:sample:coverage} \textbf{Specify intended behaviors on different kinds of input}.
It is usually not trivial to anticipate all possible input patterns, include them in the positive training examples, and define desired behavior for each.
%Even among the eligible inputs, it is usually nontrivial to foresee all possible input patterns, include them in the training examples, and define desired behaviors for them.
Therefore, we value demonstrative examples that demonstrate patterns different from the existing examples. 
%our training examples need to further articulate two things: (1) to include enough sub-groups of inputs (involving corner cases) to improve the function coverage, (2) to articulate intended behaviors on different sub-groups.



\item \label{scattershot:sample:diverse} \textbf{Avoid repetitive patterns}.
There are only a limited number of in-context demonstrations allowed in LLMs due to their computational costs.
Therefore, we should avoid wasting budget on repetitive patterns.
In \sysname's iterative setting, this also means specifying a stop condition, where the user can dynamically determine whether a function is satisfying without adding any more in-context examples.
\end{enumerate}

To support these specificity needs, we design \sysname to use LLMs for two purposes:
(1) It ranks and selects diverse unlabeled examples that can help specify function applicability and coverage, and 
(2) it proposes automatic labels for the selected candidate examples that help people to judge the quality of the current in-context function, and to consider creative labeling patterns they might have missed.
Below, we first describe how a human user can interact with \sysname, and then explain the underlying workflow, where we select the candidate examples in an active learning style approach.


\begin{figure*}[t]
\centering
\includegraphics[trim={0cm 18cm 16cm 0cm}, clip,width=1\linewidth]{figures/ui}
\vspace{-5pt}
\caption{
The \sysname interface, with (A) task description, (B) existing in-context examples, and (C) candidate examples awaiting human inspection. 
(D) Users can make edits to LLM outputs, sort the candidates into positive demonstrative examples (+), negative ones (-), or just not include the candidate (O).
The description and the examples get transformed to raw text prompts.
One set of in-context example produces multiple prompts depending on how the examples are ordered; (E) shows a prompt with one possible ordering.
}
\vspace{-5pt}
\label{scattershot:fig:ui}
\end{figure*}

\subsection{Interactive Interface}
We present \sysname as an intuitive interactive interface as shown in Figure~\ref{scattershot:fig:ui}.
The interface starts with a task description (Figure~\ref{scattershot:fig:ui}A) and existing in-context learning examples each presented as an input-output pair (B).
Both the description and the examples are editable, and are automatically translated to a prompt for driving the LLM.
As in Figure~\ref{scattershot:fig:ui}E, the prompt starts with the task description, then involves a series of example pairs in the same format of \texttt{>> [example input] => [example output]}, then \texttt{>> [candidate input] =>}, so the LLM can provide the potential output.

Below existing examples, \sysname uses a LLM to propose a batch of candidate examples for users to verify and provide feedback (C). 
%\feedback{WE provide?  Does we mean the system or you and coauthors?  Say instead “scattershot uses a LLM to propose” or something.  (next sentence says this, so you could combine them)}
These candidate examples are displayed the same way as training examples. 
%but the outputs are automatically provided by the LLM. 
Users have the options to edit the model outputs (\eg changing from \exinline{xmas == 12-25} to \exinline{xmas == 2014-12-15}), and adding examples to (or removing them from) the in-context training set  (D).
Notably, to help specify applicability, \sysname allows users to include not only positive examples (\ie eligible inputs and their desired outputs), but also negative examples (\ie ineligible inputs and a placeholder output \exinline{N/A}).
Besides taking human feedback, we also use the candidate set to implicitly support users self-assessing the quality of the current in-context dataset/function: If all unedited LLM outputs seem reasonable on some consecutive batches of selected candidates, it is likely that the in-context examples have achieved reasonable coverage, and that users can decide to terminate the iteration process.

The interface is mostly task-agnostic such that it can be generalized to various use scenarios that involve one-on-one mapping between inputs and outputs.
It can be easily invoked in Jupyter Notebook and therefore can seamlessly support users' natural workflow.




\begin{figure*}[t]
\centering
\vspace{-15pt}
\includegraphics[trim={0cm 8.5cm 8cm 0cm}, clip,width=1\linewidth]{figures/selection}
\vspace{-15pt}
\caption{
A high level overview of \sysname's slice-based sampling. 
We use the data status in the $i-1$-th iteration to perform sampling for the $i$-th iteration:
(A) we use the already LLM- or human- assessed examples to infer data slices represented as templates and estimate how the current in-context function performs on different slices;% (the same way we assess LLM correctness in (D));
(B) we use these templates to partition the unlabeled data space into various groups (phrases that match the templates are \uline{underlined});
(C) we sample unlabeled examples based on their corresponding slice size and estimated accuracy, to prioritize sampling from more uncertain and larger slices; 
(D) we run the current in-context function on the selected inputs, and deem the function correct, if prompts with different in-context example orders produce the same output. An example will only be surfaced to the interface for human inspection if the function is incorrect on it (annotated with the orange dot).
\todo{outdated, change the writeup}
}
\vspace{-20pt}
\label{scattershot:fig:selection}
\end{figure*}



\subsection{Data Slice based Sampling}


Underlying the interface, the key idea of \sysname is to select candidates that are non-repetitive, diverse, and worth human feedback.
In essence, it is an active learning problem~\cite{settles.tr09, tran2019bayesian} where a model dynamically queries an annotator for the desired output for these selected examples, so that the model can improve its performance using the updated training data.
%It is essentially an active learning problem~\cite{settles.tr09, tran2019bayesian}, where a model dynamically  query a human annotator (an  ``oracle'') to label these data points with the desired output, such that the model can improve its performance using the updated training dataset.
%However, two challenges make it difficult to directly apply an active learning algorithm.
%First, the data selection strategy for LLMs is not straightforward. 
One typical strategy is uncertainty sampling, \ie to prioritize examples that the model is least certain how to label according to model confidence or the entropy of all possible labelings~\cite{lewis1994sequential}.
Due to the generative nature of LLMs, there are an indefinite number of possible outputs (or labels), making it harder to estimate model confidence.
Even if we can measure the confidence, it is still too computationally expensive to run the LLM on every candidate input. 

As a workaround, we try to estimate how an in-context function will respond to \emph{a group of} similar examples instead of individual ones, through slice-based~\cite{chen2019slice} sampling.
By dividing the data space into subsets based on inter-instance similarities, we estimate how well the current in-context function is performing per slice, and we prioritize selecting and labeling data points from slices that haven't yet been learned.
More formally, as we iteratively select our in-context examples, at the $i$-th iteration, we split the current unlabeled data space $\mathbf{X}^u_i = \{x_1, ..., x_n\}$ into a series of $m$ automatically inferred data slices $\mathbf{S}_i = \{S_{i,1}, ..., S_{i,m}\}$.
We estimate the data slice accuracy on slice $j$, $A_{i,j} \in [0, 1]$, using the samples processed in the previous two iterations. 
Given an unlabeled input $x$ that belongs to a certain slice $x \in S_{i,j}$, we assign its probability of being sampled proportional to the estimated performance $A_{i,j}$ (such that we prioritize uncertain examples), multiplied by the size of the slice $|S_{i,j}|$ (to encourage coverage of the unlabeled space $X^u_i$):
$P(x) \propto |S_{i,j}| \cdot (1 - A_{i,j})$.
We further filter the select-to-label examples, $\mathbf{L}_i$, by estimating in-context function correctness on them, and present examples that are worth human feedback, as well as the LLM-proposed labels, in the interface.

The slice-based approach can be viewed as uncertainty sampling of different input types. It addresses the aforementioned design rationales, \ie interactively identifying data slices helps specify the function applicability, and prioritizing unlearned data slices alleviate the risk of wasting the labeling budget on repetitive patterns.
Below, we introduce how to infer the slices $\mathbf{S}_i$, estimate slice performances, and filter selected examples by correctness. 


\textbf{Infer data slices}.
Perhaps the most straightforward way would be to automatically cluster the unlabeled input examples based on their similarities.
However, empirically, we see that vanilla similarity measurements cannot help reveal meaningful slices.
For example, if we run clustering based on cosine similarities in the input sentence embedding space~\cite{reimers-2019-sentence-bert}, then \exinline{Photo: Today.} is considered closer to \exinline{Photo: on Flickr.} (similarity score $s = 0.48$) than to \exinline{Are you going to yoga today?} (similarity score $s = 0.29$), though the latter shares the key temporal phrase of ``today''.
As an alternative, we propose to estimate slices more explicitly using heuristically created templates, similar to the Snorkel labeling functions~\cite{ratner2016data}.
We collect all the inputs that have been sampled (and thus processed by the LLM) up until iteration $i-1$, extract trigrams from the sentences, and select representative templates using Tempura~\cite{wu2020tempura} -- so both \exinline{Photo: Today.} and \exinline{Are you going to yoga today?} can be put in a cluster of \exinline{today}.

We then sort the unlabeled data points into slices.
If an unlabeled input $x \in \mathbf{X}^u_i$ contains a phrase that matches with a template $t_{i,j}$, then we say $x$ belongs to the corresponding slice $S_{i,j}$.
If $x$ is not matched with any of the $m$ templates, then it belongs to a single, unsorted slice of $S_{i,m+1}$.


Note that to further eliminate potential noise in extracting trigram templates, we take advantage of the nature of our perturbation tasks, and only use trigrams in the \emph{key phrases}.
Given a labeled, positive example, \ie a pair of original and perturbed sentences $(x,y)$, we deem the edited phrases of $x$ to be key to the task, if most $x$ remain unchanged (Levenshtein edit distance $d \leq 0.5$), and the remaining phrases to be key otherwise.
For negative examples where the output would be a plain \exinline{N/A}, we simply use the full sentence as the key phrase.


\textbf{Estimate data slice performance}.
The first step to quantifying the performance of an in-context function on a data slice is to determine when a function is considered correct on a single, unlabeled input.
To do so, we take inspiration from Quey-by-Committee~\cite{melville2004diverse} and the unanimity principle~\cite{khani2016unanimous}.
Specifically, following \citet{lu2021fantastically}'s observation that the order of the same in-context examples can drastically change LLM performances, we form three different prompts by randomly reordering the examples, and get three outputs accordingly.
We only consider the current in-context function \emph{correct-by-unanimity} on an input $x$, when multiple different prompts formed with the \emph{same} in-context examples predict the same output.

To track the most recent progress, we estimate model performance using the examples processed in the last two iterations. 
We deem an example $x \in \mathbf{L}_{i-1} \cap \mathbf{L}_{i-2}$ correct, if it is correct-by-unanimity, or the human annotator did not interact with $x$'s candidate output in the interface, indicating $x$ has passed the manual inspection.
We update the performance of the corresponding slices $\{s_{i,j} | x \in s_{i,j}, x\in \mathbf{L}_{i-1} \cap \mathbf{L}_{i-2} \}$ based on these correctness.

\textbf{Filter selected examples by correctness}.
To maximize the utility of human inspection, we further filter the current samples $L_i$ using correct-by-unanimity, and only present the examples to humans if the outputs from the three prompts disagree. 
We choose the output with the minimum perplexity score as the LLM-provided, candidate label.


\begin{comment}
Finally, we use the estimated accuracy for sampling.

By computing the editing operations, we can extract the key phrases important to a specific perturbation function, and compute semantic diversity directly on the key phrases.
For all the existing few-shot examples, we compute the edited snippets on each {orig, perturbed} pair, convert the edit to templates, so eventually each template can be seen as a set of perturbation pairs: t = {(o1, p1), (o2, p2), …}




(\eg )
(), since 
Here, we 

By computing the editing operations, we can extract the key phrases important to the specific task, and compute semantic diversity directly on the key phrases.

This is similar to automatically extracting labeling functions~\cite{}.

Second, we need to \emph{estimate function performance on each data slices}.

With these two information, we can perform weighted sampling


That is, we infer data slices based on 
Intuitively, improving performance on application-critical data subsets, or slices

It’s a bit similar to automatically extracting some snorkel labeling functions. The assumption is that if some cases are not covered by patterns extracted from current few-shot examples, then it makes sense to prioritize them.







we deem an example difficult and ``unknown'' to the current in-context function, if different subsets of the existing training examples drive LLMs to produce inconsistent outputs.


unlike most active learning literature on classification tasks where there is a fixed set of possible outputs, it is less clear how to measure LLM certainty in a generative space.


Sample, penalize, or reward candidate data points by estimated accuracy on corresponding data slices.
Start with unweighted sampling: give all the candidate, unlabeled examples equal probability of getting selected = 1
Estimate data slices: compute data slides templates based on last three batch
Estimate data slides success rate, based on text overlaps between full few-shot output, and subgroup few-shot outputs. A data slice is “learned” if its estimated accuracy > 0.8; unlearned if < 0.5.


find other slices *only if* we know the current slice is solved, using a similar method as uncertainty sampling. Try estimating accuracy dynamically (e.g. through GPT-3 output uncertainty), and penalize certain slices only when the estimated accuracy in the last two iterations > a threshold.


\feedback{but how does scattershot recognize inconsistent results (indeed, what does this mean?) do you mean inconsistent or just variable as in changing the set of training examples causes SS to change the prediction somehow?  (I guess the latter given your text overlap metric lower). That doesn’t match ‘inconsistency’ in my book; instead it seems more like uncertainty or instability.  (I do think it makes sense to connect the idea or intuition to uncertainty sampling in active learning.) I’d also consider the name ‘instability sampling'}
%To help improve coverage on different sub-types and corner cases, we design a 
Taking inspiration from \citet{khani2016unanimous}, we deem an example difficult and ``unknown'' to the current in-context function, if different subsets of the existing training examples drive LLMs to produce inconsistent outputs.
Figure~\ref{scattershot:fig:selection}A demonstrates the intuition behind such a setup: 
on the input \exinline{[Posted: 2014-03-30] Last day to get extra \$10 at http://t.co/YKw31KI7ES!}, different subsets of existing in-context learning examples drive the LLM to generate three drastically different outputs: \exinline{http://t.co/YKw31KI7ES == 2014-03-30}, \exinline{N/A}, and  \exinline{\$10 == 2014-03-30}, essentially indicating that the supposed behavior on the given input has yet to be learned.
Asking people to inspect and fix the LLM output on this input can be a valuable complement for stablizing model behaviors.
Meanwhile, an stable output of \exinline{23.03.2015 == 2015-03-23} in Figure~\ref{scattershot:fig:selection}B indicates that the existing in-context examples are sufficient for the LLM to process this input, and that further adding it could be inefficient.


More specifically, as in Figure~\ref{scattershot:fig:selection}, we split the existing training set through three-fold, so we have three ``versions'' of current functions, $F_1$, $F_2$, $F_3$, with slightly different in-context examples.
For each input, we collect up to two sampled outputs per function, forming an output set of up to six examples, and we estimate consistency by the average text overlap.
Empirically, we deem an input example to be potentially valuable if the resulting output text overlap is lower than 0.7.
Among these candidate outputs, we select the one with the highest sentence probability from LLM to show to the humans.

However, this method creates a caveat: it would also filter out ``unknown unknowns''~\cite{lakkaraju2017identifying} --- examples where all subsets of training examples are consistently wrong --- making it hard to recover from certain errors like spurious correlations with high confidence.
%\feedback{Ok to draw this connection, but it’s also a well known weakness of uncertainty sampling.}
Figure~\ref{scattershot:fig:selection}C shows such an example, where all subset functions consistently omit the year when normalizing \exinline{Sep}.
As a walkaround, even for examples with consistent outputs, we assign a probability of $p=30\%$ to display them to the user.
%\feedback{The way I think about this is your UI is creating a mixture of  two distributions of examples to show the user. (Really not cleart how much or often this is helping. In an ideal world, one would do an experiment / user study to see whether showing only unstable examples is better than also throwing in other examples with p=.3 – or better optimizing the probability with which you choose those examples.  This latter step would be hard to do, of course, because it would be very problem specific, but what you are doing with the P=.3 seems incredibly ad hoc.}
\end{comment}

==> backups/relate__.tex <==
\section{Background and Related Work}

\begin{comment}

Models in the Loop: Aiding Crowdworkers with Generative Annotation Assistants


Note – related work from Yejin and Noah: WANLI: Worker and AI Collaboration for Natural Language Inference Dataset Creation, human-in-the-loop NLI example generator, they show training with generated examples is going to improve performance on challenging datasets like HANS. 
Find challenging phenomenon through some embedding clustering
Over-generate examples from GPT-3, both premise and hypothesis
Use uncertainty between multiple NLI model checkpoints to get examples that should be labeled 
Ask human to optionally revise the generated example and label 
Compare: the uncertainty selection is a bit similar, but they don’t have applicability problem
Not technical, but if we can characterize cases where interaction works the best, I think that would also be a contribution.

NLP papers: 
specific generators are hard to meet user requirements on arbitrary perturbations; 
Few-shot learners like GPT-3 require people to come up with diverse examples;
There are papers extracting few-shot examples from *existing datasets* or for classification tasks, but we target at *generating* potentially useful examples.

HCI / PBD papers (e.g. Wrangler): 
more structured (and related work for Excel applications, table data, or syntactic text rewriting), and usually don't need to search for test/new training cases; 


We explore building in-context learning functions for generative tasks together with GPT-3. This is a training example search in an unlabeled space, generative space.  So the example search is unique:
Diverse examples that can test generalizability. This is in-contrast to searching few-shot examples in labeled tasks, where we can rely on some known development set.
Applicable examples that have the potential to be “labeled” / edited by the potential function. 
Almost-there examples, i.e. GPT-3 generated “labels” are worthy of/ can inspire human revision. If GPT-3 edit is totally off then humans wouldn’t want to add these examples, and if they are totally correct then adding these examples would not be helpful. This is in contrast to PBD, where new examples are always pruning the function search space & people only need to point out what’s wrong; Here humans really need to create the correct example. 

These are also especially hard given the generative nature of the task. If it gives 3 drastically different ”labels”, it’s hard to know if (1) all of these are right (e.g., synonym replacement at different tokens), (2) all of them are incorrect and not fixable, or (3) some of them are correct or at least fixable.

## use model as labeler

\end{comment}


% \todo{Add a section on LLM in general, possibly similar to the AI chain paper}
% 
%\paragraph{Example selection.}


% select example that's most similar to a given instance, and usually in a fully labeled space
% or select for diversity, but diversity is surface levelxtte\

% \textbf{Large Language Models.}
\subsection{An Introduction to Large Language Models and In-context Learning} 
Transformer-based large language models (LLMs)~\cite{vaswani2017attention} have recently led to large improvements in NLP.
Pre-trained on a large amount of unlabeled text data, these models encapsulate rich,  general-purpose features of language both syntactically and semantically. 
These features can help facilitate various downstream applications much more dynamically~\cite{liu2021pre} --- rather than having to train a new model for every custom task, users can just customize the model by feeding it natural language \textbf{prompts} at run time, like the holiday in the previous section. 
Such ability of recognizing the desired task on-the-fly is called \emph{in-context learning}~\cite{brown2020language}. 

The flexibility of in-context learning intrigues various works on exploiting LLMs' in-context learning capability, by designing prompts is imperative to invoke the user desired functionalities~\cite{min2022rethinking, xie2021explanation, rubin2021learning}. 
To date, the most common patterns for prompting are either \emph{zero-shot} or \emph{few-shot} prompts.
Zero-shot prompts directly describe what ought to happen in a task: \eg we can enact the holiday date  translator with a \emph{task description} prompt: \exinline{Identify the date for a national holiday in the MM-DD format.}
In contrast, \emph{few-shot} prompts show the LLM what pattern to follow by feeding it examples of the desired input and output data.
As can be seen above, given examples on \exinline{Christmas} and \exinline{Halloween}, the LLM would produce a reasonable date for \exinline{Independence Day}.
These examples usually follow consistent structures with meaningful prefixes (\exinline{Holiday: [name] => Date: [date]}), which helps re-emphasize the desired intent~\cite{vaswani2017attention}.

Despite the potential of in-context learning, the usefulness of a learned function heavily relies on the five to thirty in-context examples that demonstrate the intended behavior~\cite{rubin2021learning, lu2021fantastically}. 
If developers omit corner cases in the few examples they created, the task quality can easily be affected~\cite{liu2022wanli}.
For example, without a negative example where we denote ineligible inputs with a placeholder output \exinline{N/A} (\exinline{Holiday: yesterday => Date: N/A}), the LLM would attempt to produce the most plausible ``label'' even for negative examples --- It may try to normalize
\exinline{yesterday} to a most plausible date even though there is no \emph{holiday}.

Our work here tries to help users interactively identify high quality in-context examples for text transformation.

\subsection{}



\paragraphBold{Auto-searching Demonstrative Examples.}
Considering the importance of in-context prompts quality, various studies, therefore, focus on \emph{prompt engineering}~\cite{lu2021fantastically, betz2021thinking, liu2021makes}. Strategies like progressive generation (\ie multi-round text expansion)~\cite{tan2020progressive} and meta-prompting (\ie asking the model to elaborate on the problem)~\cite{betz2021thinking, reynolds2021prompt} attempt to seed LLMs to generate more effective prompts before solving the task.
% 
Nevertheless, as manual prompting and prompt generation can be sub-optimal, a line of studies resort to obtaining prompts by automatically selecting more effective prompts from datasets. 
% 
A body of prior work simply applies random sampling to select the labeled examples to compose the in-context prompts~\cite{chang2021neural,li2021prefix,chang2020dart}. They show that sampling tends to help identify informative examples because pre-trained LLMs possess high-level semantic features~\cite{tamkin2022active}.
Further, many studies try to optimize for \emph{local} performance, \eg dynamically selecting the most similar demonstrations for each given input~\cite{liu2021makes}, which requires searching and selecting in-context examples from fully labeled datasets~\cite{rubin2021learning, wang2021want, zhao2021lmturk}.



In the unlabeled search space, previous studies try to allocate an annotation budget to find out the most representative training data.
% based on training data diversity. 
Given a budget, an active learner iteratively selects examples-to-annotate from an unlabeled pool according to some ranking mechanism.
For instance, \citet{chang2021training} presents a simple selection strategy with K-means clustering to choose the diverse and representative instances of the entire data distribution~\cite{sener2017active}.
\citet{eyuboglu2022domino} proposes the Slice Discovery Method (SDMs) to automatically identify data slices that are both underperforming for models and coherent (\ie united by a human-understandable concept).
% data slices that are particularly challenging to models.
% 
Besides, \citet{liu2022semantic} introduce Semantic-Oriented Unlabeled Priming (SOUP), a method that classifies examples by retrieving semantically similar unlabeled examples, assigning labels to them in a zero-shot fashion, and then using them for in-context learning.
% 
% 
In addition, example creation and selection are also commonly seen in programming-by-demonstration (PBD).
For example, \citet{zhang2020interactive} explored effectively selecting examples that can help disambiguate and validate synthesized regular expressions.
% 
% 
In essence, these approaches also adopt the spirit of multi-step problem solving, but focus on expanding the context \textit{without} human intervention.
% 
However, the mined prompts tend to be less human-readable~\cite{shin2020autoprompt} and there is a lack of quantitative evaluation criteria to assess the data quality rigorously~\cite{eyuboglu2022domino}, thus less compatible with human-AI interaction. Therefore, it is essential to select examples that incentivize people to provide feedback.
% 
We share similar motivations that interactively and iteratively suggest corner cases help synthesize the right function, but unlike PBD where new examples are always \emph{pruning} the function search space, ScatterShot focuses on \emph{expanding} the function coverage and encouraging example diversity~\cite{sener2017active} in the human-AI interaction scenarios.
% \todo{eyuboglu2022domino}\hua{no problem!hhhh}






\paragraphBold{Active Learning with Human Interaction.} 
Interactively sampling and selecting a small subset of informative examples by humans can be viewed as active learning for in-context learning~\cite{settles.tr09, tran2019bayesian}, where the models can interactively query an oracle (\eg a human annotator) to label new data points with the desired outputs~\cite{settles2009active}. 
% 
The key idea behind active learning is that machine learning models can achieve higher performance with fewer training examples, if it is allowed to choose its own, most informative training examples.
% 
Prior studies have explored leveraging pool-based active learning to speed up BERT fine-tuning while keeping the cost of labeling new data constant
\cite{griesshaber-etal-2020-fine}. However, there is a lack of work investigates how humans can use active learning to craft prompts for LLMs during in-context learning.
% 
Especially, our method is closer to uncertainty sampling for active learning~\cite{lewis1994sequential}, where an active learner queries the instances about which they are least certain to label, which aims to reduce the annotation cost~\cite{raj2022convergence,sharma2017evidence}.


In addition, existing active learning studies commonly select pool-based unlabeled examples and ask humans to annotate given pre-defined labels~\cite{monarch2021human,tran2019bayesian}. Scattershot enables humans to flexibly modify the in-context examples and LLMs to generate unseen outputs. This advantage can potentially compensate for user omissions~\cite{ross-etal-2022-tailor, lee2022coauthor}, help humans complete tasks more effectively~\cite{wang2021want, wu-etal-2021-polyjuice}, and is specifically effective for human ideation: they can introduce new characters into human-generator co-written novels~\cite{lee2022coauthor}, and can exploit specific linguistic patterns and enrich otherwise rare data types~\cite{liu2022wanli}.
These works mostly use generators for ideating \emph{instances}, with the assumption that the task itself (\eg novel creation, dataset expansion) is clearly defined.
Our work more explicitly explore the gains from \emph{concept} ideation, or how much LLMs can help people refine their task specification.
% 
Importantly, while many empirical results suggest that active learning is effective, it does suffer from certain limitations. For example, the labeled examples are not drawn i.i.d  from the underlying data distribution~\cite{settles.tr09}, and therefore can sometimes be imbalanced~\cite{pop2018deep} or less effective than random sampling~\cite{imberg2020optimal}.
Our method will likely share the same limitations, though we leave it to future work to articulate scenarios where ScatterShot is most useful. 






% \textbf{Generators for inspirations.}
% Prior work has shown that generators can potentially help humans complete tasks more effectively~\cite{wang2021want, wu-etal-2021-polyjuice}, and compensate for their omissions~\cite{ross-etal-2022-tailor, lee2022coauthor}.
% Generators seem specifically effective for ideation
% : they can introduce new characters into human-generator co-written novels~\cite{lee2022coauthor}, and can exploit specific linguistic patterns and enrich otherwise rare data types~\cite{liu2022wanli}.
% These works mostly use generators for ideating \emph{instances}, with the assumption that the task itself (\eg novel creation, dataset expansion) is clearly defined.
% Our work more explicitly explore the gains from \emph{concept} ideation, or how much LLMs can help people refine their task specification.
% 
% Importantly, while many empirical results suggest that active learning is effective, it does suffer from certain limitations. For example, the labeled examples are not drawn i.i.d  from the underlying data distribution~\cite{settles.tr09}, and therefore can sometimes be imbalanced~\cite{pop2018deep} or less effective than random sampling~\cite{imberg2020optimal}.
% Our method will likely share the same limitations, though we leave it to future work to articulate scenarios where ScatterShot is most useful. 





%\feedback{Section 5.5 need some discussion of active learning – can point out that it is traditionally cast as selecting an unlabeled example, instead of GENERATING one – but still need something.  A very cursory look (you should look much more) includes: https://proceedings.mlr.press/v97/tran19a/tran19a.pdf}








% ===================== dead kitten =====================
\begin{comment}



% Our method is closer to uncertainty sampling~\cite{lewis1994sequential}, where an active learner queries the instances about which it is least certain how to label.
% Note that because LLMs are generative in nature and do not have clear probabilistic distributions across all ``labels'' as in \eg classification tasks, we estimate uncertainty using the LLM output stability: if  different prompts ``vote'' for different outputs, then we say the LLM is uncertain about the corresponding input given the current few-shot examples.
% This voting strategy is also quite relevant to Query-By-Committee~\cite{seung1992query} where a list of ``committee'' models trained on the same labeled set vote on the labelings of query candidates.


% Active learning
% to sampling approaches in active learning.
% Indeed, the selection part of our work can be seen as active learning~\cite{settles.tr09, tran2019bayesian} for in-context learning.

% The key idea behind active learning is that machine learning models can achieve higher performance with fewer training examples, if it is allowed to choose its own, most informative training examples.
% 
% 
% In contrast, our work focuses more on an unlabeled space, and as a result focuses more on \emph{iterative task definition}.



% \hua{I would probably replace this paragraph of ``Generators for inspirations'' with ``active learning'' and ``human prompting''. The reason is ``Generators for inspirations'' is discussing the human+LLM effects on human tasks, whereas our project is about human + LLM for improving LLM tasks. This goal is closer to ``active learning'' and ``human prompting''}

% \todo{blind spot detection methods}





% Aside from the prompt itself, we also associate with each LLM operation a default \textbf{temperature setting}: a model parameter that influences the randomness of the LLM generation.
% For instance, creative operations like \emph{Ideation} benefit from a higher temperature ($t\text{=}0.7$) than  more factual or deterministic tasks like \emph{Classification} ($t\text{=}0.0$)~\cite{gpt3instruct}.






% Prior work has explored selecting effective demonstrations, and has shown that because pre-trained models possess high-level semantic features, sampling or active learning tend to help identify informative examples~\cite{tamkin2022active}.
% 
% Many of these studies tries to optimize for \emph{local} performance, \ie dynamically selecting the most similar demonstrations for each given input~\cite{liu2021makes}, which requires searching and selecting in-context examples from fully labeled datasets~\cite{rubin2021learning, wang2021want, zhao2021lmturk}.

% As manual prompting can be sub-optimal, some work automatically mines more effective prompts.

% Conversely, strategies like progressive generation (\ie multi-round text expansion)~\cite{tan2020progressive} and meta-prompting (\ie asking the model to elaborate on the problem)~\cite{betz2021thinking, reynolds2021prompt} attempt to seed LLMs to generate more effective prompts before solving the task.


% Following this convention, this study builds the prompts to include 
% we build our prompts to include \emph{task descriptions} followed by \emph{prefixes}.




% 
% 
% 
% 
% \textbf{Selecting demonstrative examples.}
% \hua{\textbf{Auto example search}}
% In-context learning has been shown to heavily depend on the demonstrative, ``training'' examples, and LLMs can only perform in-context learning if it has seen the corresponding distribution or concept~\cite{min2022rethinking, xie2021explanation, rubin2021learning}. 

% Prior work has explored selecting effective demonstrations, and has shown that because pre-trained models possess high-level semantic features, sampling or active learning tend to help identify informative examples~\cite{tamkin2022active}.
% Many of these studies tries to optimize for \emph{local} performance, \ie dynamically selecting the most similar demonstrations for each given input~\cite{liu2021makes}, which requires searching and selecting in-context examples from fully labeled datasets~\cite{rubin2021learning, wang2021want, zhao2021lmturk}.




% % 
% % 
% \sherry{
% Semantic-Oriented Unlabeled Priming for Large-Scale Language Models
% % 
% "We introduce Semantic-Oriented Unlabeled Priming (SOUP), a method that classifies examples by retrieving semantically similar unlabeled examples, assigning labels to
% them in a zero-shot fashion, and then using
% them for in-context learning."
% => can compare and say it's impossible to auto label generative tasks
% }



% \citet{chang2021training} has tried to allocate an annotation budget based on training data diversity akin 




% In the unlabeled search space, \citet{chang2021training} has tried to allocate an annotation budget based on training data diversity akin to sampling approaches in active learning.
% Indeed, the selection part of our work can be seen as active learning~\cite{settles.tr09, tran2019bayesian} for in-context learning.
% The key idea behind active learning is that machine learning models can achieve higher performance with fewer training examples, if it is allowed to choose its own, most informative training examples.
% Given a budget, an active learner iteratively selects examples-to-annotate from an unlabeled pool according to some ranking mechanism.
% In \citet{chang2021training}'s case, the examples are selected through diversity~\cite{sener2017active}; However, diversity is usually ill-defined for various tasks~\cite{rubin2021learning}.




% In addition, example creation and selection is also commonly seen in programming-by-demonstration (PBD).
% For example, \citet{zhang2020interactive} explored effectively selecting examples that can help disambiguate and validate synthesized regular expressions.
% We share similar motivations that interactively and iteratively suggesting corner cases help synthesize the right function, but unlike PBD where new examples are always \emph{pruning} the function search space, ScatterShot focuses on \emph{expanding} the function coverage.
% Therefore, it is essential to select examples that incentivize people to provide feedback.

% \hua{combine \textbf{blind spot detection methods} with demonstrative examples searching.}


% % 
% % 
% \sherry{
% Semantic-Oriented Unlabeled Priming for Large-Scale Language Models
% % 
% "We introduce Semantic-Oriented Unlabeled Priming (SOUP), a method that classifies examples by retrieving semantically similar unlabeled examples, assigning labels to
% them in a zero-shot fashion, and then using
% them for in-context learning."
% => can compare and say it's impossible to auto label generative tasks
% }



% In \citet{chang2021training}'s case, the examples are selected through diversity~\cite{sener2017active}; However, diversity is usually ill-defined for various tasks~\cite{rubin2021learning}.




\end{comment}

==> backups/simulation.tex <==

\section{Simulation Experiment: \sysname Sampling vs. Random Sampling}
\label{sec:simulation}

\begin{figure*}
\centering
\includegraphics[trim={0cm 15.5cm 18cm 0cm}, clip,width=1\linewidth]{figures/ui_qa}
\vspace{-10pt}
\caption{
(A) The \sysname interface, with (A$_1$) task description, (A$_2$) existing in-context examples, and (A$_3$) candidate examples awaiting human inspection. 
Through interactions A$_4$ and A$_5$.
Users can make edits to LLM outputs, sort the candidates into positive demonstrative examples (+), negative ones (-), or just not include the candidate (O).
The description and the examples get transformed to raw text prompts.
One set of in-context example produces multiple prompts depending on how the examples are ordered; (B) shows a prompt with one possible ordering.
}
\vspace{-5pt}
\label{fig:ui_qa}
\end{figure*}

We quantify the effectiveness of \sysname via preliminary case studies on two tasks. 
We first use a temporal expression normalization task to estimate whether the \sysname-learned functions are high quality enough.
Then, we also describe qualitatively how \sysname aids humans to articulate their desired functions, through another task of perturbation function creation. 

\subsection{Case 1: Temporal Expression Extraction and Normalization}

The task relates to data wrangling~\cite{verbruggen2021semantic}, and concerns extracting phrases with temporal meaning from sentences or documents, and normalizing them into standard formats~\cite{chang2012sutime}.
As shown in Figure~\ref{scattershot:fig:teaser}, these temporal expression can include absolute dates or dates relative to a reference (\eg post date), and can have different granularity (\eg exact date vs. year only).
%\feedback{does this mean that you eliminate all negative examples, ie those with no time expressions? I guess so.  Probably worth justifying why. What would have happened to your results if you had left the hard examples?  Are you going to distribute the new dataset? Say how to get it, eg point to an appendix or repo. If not, why not?}
We take the data from \cite{almasian2021bert}, which contains common temporal datasets including TimeBank~\cite{pustejovsky2006timebank} and TweeTime~\cite{tabassum2016tweetime}, containing temporal expression annotations on news articles and tweets, respectively.
This fully labeled dataset enables us to simulate a labeling process with an oracle that always provide groundtruths. 
Moreover, by evaluating the in-context function on holdout sets, we are also able to quantify the learned function quality.

Since some of the normalizations are arguably ambiguous and hard to control, we process the dataset such that (1) we only kept data points that could be normalized to the format of YYYY-MM-DD, and (2) we split long documents into single sentences, and only kept sentences that involve absolute dates, or describe dates relative to the document publication date, or no time expression at all (as the pool for negative examples).
We collected 491 positive examples and 369 negative ones this way.
\footnote{The processed data can be found in \url{https://github.com/tongshuangwu/scattershot-data}.}
We randomly sample 100 positive and 50 negative examples to form the test set, and use the remaining examples as a pool for selecting in-context examples.

\textbf{Procedure and baseline.}
We take advantage of the gold labels, and design a simulation study comparing \emph{\sysname} with a \emph{Random} baseline where we replace the slice-based sampling with plain random sampling.

The simulation setup for both systems is the same, and the gold labels are used as the oracle labeler.
The process starts with three random seeding examples, and in each iteration, we compare the gold label with the LLM-proposed candidate label.
If these two labels differ, we add the pair of (input, oracle output) into the in-context example set, simulating the case where the human annotator corrects the LLM;
Otherwise, the oracle will not perform any action, simulating cases where humans decide to do nothing on already-learned patterns.
We repeat the process until one of the three stop conditions is met: (1) the in-context example set contains more than 30 data points, (2) the oracle labeler has been presented more than 100 examples, or (3) in two consecutive iterations, the in-context function correctly generated outputs for all the selected examples.
Once the iteration is stopped, we use the final in-context function to generate outputs for all the examples in the test set, and follow \citet{chang2012sutime}'s practice in evaluating the result. Specifically, we report the F1, recall, and accuracy for both the time expression extraction and the normalization.
We repeat the procedure three times for more stable observation.





\begin{table*}
\small
\centering

%\renewcommand{\arraystretch}{0.85}
\setlength{\tabcolsep}{1pt}

\begin{tabular}{@{}r c c c c c c @{}}
\toprule

\multirow{3}{*}{Conditions}
& \multicolumn{3}{c}{\textbf{Extraction}} & \multicolumn{3}{c}{\textbf{Normalization}} \\
\cmidrule(lr){2-4}
\cmidrule(lr){5-7}
& F1 & Precision & Recall & F1 & Precision & Recall \\
\midrule\midrule
Random &  72.3 $\pm$ 4.4 &  73.6 $\pm$ 4.2 &  72.5 $\pm$ 4.5 &  66.9 $\pm$ 3.3 &  67.6 $\pm$ 3.6 &  67.1 $\pm$ 3.1 \\
\sysname & \textbf{ 76.1 $\pm$ 3.6} & \textbf{ 76.8$\pm$ 3.5 } & \textbf{ 75.8 $\pm$ 3.7} & \textbf{ 71.1 $\pm$ 3.1 } & \textbf{71.6 $\pm$ 3.3} & \textbf{ 71.4 $\pm$ 3.0} \\
\bottomrule
\end{tabular}
\centering
% \vspace{-5pt}
\caption{
Quantitative results comparing \sysname with random baseline on temporal expression, averaged over 10 random seeds.
\sysname outperformed the baseline on all metrics.
% 
}
%\vspace{-10pt}
\label{scattershot:tab:temporal}
\end{table*}






\begin{table*}
\small
\centering

%\renewcommand{\arraystretch}{0.85}
\setlength{\tabcolsep}{9pt}

\begin{tabular}{@{}l c c @{}}
\toprule

\multirow{1}{*}{Conditions}
& \multicolumn{1}{c}{\textbf{Rouge}} & \multicolumn{1}{c}{\textbf{EM}} \\
\midrule\midrule
Random &  73.26 $\pm$ 4.11 &  29.40 $\pm$ 6.68 \\
\sysname & \textbf{ 77.01 $\pm$ 3.89} & \textbf{ 30.9 $\pm$ 5.33}  \\
\bottomrule
\end{tabular}
\centering
% \vspace{-5pt}
\caption{
Quantitative results comparing \sysname with random baseline on targeted text perturbation, averaged over 10 random seeds. 
\sysname outperformed the baseline on all metrics. 
% 
}
%\vspace{-10pt}
\label{scattershot:tab:temporal}
\end{table*}





\textbf{Result.}
As shown in Table~\ref{scattershot:tab:temporal}, \sysname outperforms the baseline especially on extraction. 
Note that this is a stronger baseline than asking humans to manually craft a training set, as it assumes a reasonable access to less obvious cases that humans might have missed, and it also ensures that all the labels are correct.
This suggests that \sysname has the potential to improve in-context learning function qualities. 

%\feedback{use textbf to draw attention to best numbers.  I think I’m fuzzy on the methodology. Is this right? You use SS to generate a set of 18 examples and then this is fed into the LLM and the final results are the results of the in-context trained LLM on a different test set (compared to the same LLM using fully random examples for in-context training).  If so, I missed what the actual test set was. I do think you should recap a bit of this in the caption for table 5.1, including what the test set is.How many of these examples came from the instability sampling and how many came from the P=0.3 test?   (There’s no way for me to estimate that number is there?  It depends on what percentage of the examples are unstable, right?). worth including this even if you don’t compare to a version that doesn’t use P=.3}

\begin{table*}[t]
\small
\centering

%\renewcommand{\arraystretch}{0.9}
%\setlength{\tabcolsep}{10pt}

\begin{tabular}{@{}l || r | l @{}}
\toprule
\multirow{6}{*}{\rotatebox[origin=c]{90}{Coverage}}
& Input & Q: Are there more girls or boys? A: equal \\
& Template & \emph{(Not applicable)} \\
& Random & \emph{Q: Are the girls and boys equal in number? A: yes} \\
& \sysname & Q: Are the girls and boys equal? A: yes \\
\cmidrule{2-3}
& Input & How many hairs does the sheep in front have? A: infinite \\
& Template & \emph{(Not applicable)} \\
& Random & \emph{(Not applicable)} \\
& \sysname & Q: Does the sheep in front have infinite hairs? A: yes \\
\midrule\midrule


\multirow{6}{*}{\rotatebox[origin=c]{90}{Fluency}}
& Input & Q: What does the woman have on her face? A: headband \\
& Template & Q: Does the woman have on her face headband ? A: yes \\
& Random & Q: Does the woman have a headband on her face ? A: yes \\
& \sysname & Q: Does the woman have a headband on her face ? A: yes \\
\cmidrule{2-3}
& Input & Q: What make is the phone? A: vtech \\
& Template & Q: Make is the phone vtech ? A: yes \\
& Random & Q: Is the phone a vtech ? A: yes \\
& \sysname & Q: Is the phone a vtech ? A: yes \\
\midrule\midrule

\multirow{6}{*}{\rotatebox[origin=c]{90}{Correctness}}
& Input & Q: What monument are they next to? A: unknown \\
& Template & Q: Are they next to unknown? A: yes \\
& Random & Q: Is the monument unknown? A: yes \\
& \sysname & Q: Are they next to an unknown monument? A: yes \\
\cmidrule{2-3}
& Input & Q: What type of motorcycle is in the picture? A: mountain \\
& Template & Q: Is the mountain in the picture ? A: yes \\
& Random & Q: Is the mountain type of motorcycle in the picture ? A: yes \\
& \sysname & Q: Is the motorcycle in the picture a mountain bike? A: yes \\

\bottomrule
\end{tabular}
\centering
% \vspace{-5pt}
\caption{
Example outputs from perturbation functions built in \sysname and Random condition, and from templates in \citet{ribeiro2019red} et al.
\sysname functions tend to be able to perturb more forms of inputs (``coverage''), sound more natural (``fluent''), and tend to produce desired outputs (\ie the new question-pair are logically equivalent to the original pair).
}
%\vspace{-10pt}
\label{scattershot:tab:perturb_qual}
\end{table*}

\subsection{Case 2: Targeted Text Perturbation}
\label{scattershot:case:perturbation}

We also explore using \sysname to replicate perturbation functions in prior work for evaluating NLP model behavior consistency.
Given one testing objective, researchers usually investigate a lot of manual effort to create and refine multiple templates for handling different input types.
Even with these, the templates could be too strict to generate natural texts for many intended inputs.
For example, just for testing question answering models' robustness on logically equivalent questions, \citet{ribeiro2019red} et al. created four subtly different templates that perturb based on their parsing tree structures. 
We are interested in whether \sysname can help achieve compatible or better perturbations while saving the manual effort crafting templates.
As such, we design the second case study to replicate the \emph{logical equivalence} perturbation in \cite{ribeiro2019red} with in-context learning.

\textbf{Procedure.}
While we were able to download \citet{ribeiro2019red}'s pairs of input sentences and template-perturbed outputs\footnote{\url{https://github.com/marcotcr/qa_consistency}}, the template outputs are generally noisy and therefore cannot be an oracle as in the temporal expression case.
Rather, we use the case to run a preliminary user study. 
We invited two NLP graduate students to interact with the \sysname interface and build the perturbation function for \emph{logical equivalence}.
We first briefed participants on the task by providing them with task descriptions and sample (seeding) examples. 
Then, we asked them to create in-context training sets twice, once with each condition (\sysname and Random, where again we provide ScatterShot to users without the slice-based sampling), whose orders were counterbalanced.
We asked them to spend up to 25 minutes per condition, but allow them to stop early if they are satisfied with their functions. We encouraged participants to think aloud and describe their actions as they completed the task. 

\textbf{Results.}
We took their built in-context function and ran a similar quantitative comparison as in the previous temporal expression study.
We saw that the function they built through \sysname produces more valid perturbations (\ie correct and fluent ones for 78\% of the time) than the function produced in the \emph{Random} condition (61\%).
\footnote{We resolved to manually verifying perturbations on 120 original examples because, again, the template outputs were noisy.}

Qualitatively, \emph{Random} functions contained 21 in-context examples on average whereas \emph{\sysname} ones contained 30.
This indicates that without the help of \sysname, users tended to misjudge the in-context function quality, and incorrectly stop the iteration way before the function performance converges.
As shown in Table~\ref{scattershot:tab:perturb_qual}, the use of \sysname also helped increase coverage on less apparent data slices like \exinline{how many} and \exinline{why} questions, rather than the most frequent \exinline{what} questions.

We also compared \emph{\sysname} functions with \citet{ribeiro2019red}'s original templates, and found \sysname outperformed \emph{Templates} on coverage, fluency, and correctness.
While preliminary, these results point to \sysname potential on saving human efforts in creating fine-grained functions, alleviating the need of handcrafting templates.

